Tequila: A platform for rapid development of quantum algorithms

Variational quantum algorithms are currently the most promising class of algorithms for deployment on near-term quantum computers. In contrast to classical algorithms, there are almost no standardized methods in quantum algorithmic development yet, and the field continues to evolve rapidly. As in classical computing, heuristics play a crucial role in the development of new quantum algorithms, resulting in high demand for flexible and reliable ways to implement, test, and share new ideas. Inspired by this demand, we introduce tequila, a development package for quantum algorithms in python, designed for fast and flexible implementation, prototyping, and deployment of novel quantum algorithms in electronic structure and other fields. Tequila operates with abstract expectation values which can be combined, transformed, differentiated, and optimized. On evaluation, the abstract data structures are compiled to run on state-of-the-art quantum simulators or interfaces.

==> extensions.tex <==
Extensions to \tequila are largely accomplished through the addition of new inheritors of various base classes. In the case of circuit execution, this is achieved through defining inheritors of the classes \texttt{BackendCircuit} and \texttt{BackendExpectationValue}. To add new optimizers, the \texttt{Optimizer} and \texttt{OptimizerResult} classes require new inheritors to be defined. For new quantum chemistry backends, an inheritor  \texttt{QuantumChemistryBase} is needed. Hamiltonian arithmetic backends can, in theory, be added by modifying the classes \texttt{Paulistring} and \texttt{QubitHamiltonian} should have new class methods added to them, in order to convert to and from the corresponding backend objects. \\
For full integration into the \tequila framework, it is necessary to modify certain files slightly so that global helper functions, like \textit{tq.minimize} or \textit{tq.compile} are able to access the new classes. Upon addition of new circuit execution backends, the file \textit{tq.simulators.simulator{\_}api.py} needs to have its import preamble modified; supposing a new backend package called \textsc{foobar} which supports all functionalities, the preamble addition is as follows:

\lstinputlisting[language=Python]{code/import_statements.py}

Similarly, if a new optimizer module \textsc{foobar} is added, then the file \textit{tq.optimizers.{\_}{\_}init{\_}{\_}.py} requires the following addition:

\lstinputlisting[language=Python]{code/optimizer_import_1.py}

The user also should add the string \textit{'foobar'} to the list in that same file of supported optimizers. \\

For a more concrete examples of extending \tequila, please check the instruction document on the github page.



%In the following section, we detail how  \tequila may be augmented with new backends for quantum simulation, quantum chemistry, numerical optimization, and Hamiltonian arithmetics. 

%\subsection{simulation}
%the simulation or execution of a quantum circuit is handled by classes which inherit from the BackendCircuit and BackendExpectationValue classes. To add a new circuit backend, the inheriting classes must overwrite several methods of BackendCircuit, in addition to whatever new methods may be required, and alteration of the constructor. The methods which must be overwritten are \textit{initialize{\_}circuit}, \textit{add{\_}basic{\_}gate}, \textit{add{\_}parametrized{\_}gate},  \textit{do{\_}simulate} (if supported), \textit{do{\_}sample} (if supported), and \textit{convert{\_}measurement}.
%In order to support the use of real or emulated devices, the methods \textit{check{\_}device} and \textit{retrieve{\_}device} should be re-implemented. If use of a device requires alterations to already-translated circuits, \textit{apply{\_}device} should be re-implemented. Support for noise will vary from backend to backend, but the method \textit{process{\_}noise} should be overwritten; if noise is not applied to circuits but passed handled on simulation call, note that \textit{do{\_}sample} must account for this. \\

%While entirely optional, some further alterations to the base class are advisable to increase efficiency. The dictionary attribute \textit{compiler{\_}args} should be re-written so that any unnecessary conversions are set to false, to speed up initialization. Furthermore, if the simulation backend has some internal structure that handles parametrization, the methods \textit{process{\_}variables} and  \textit{update{\_}variables} \\

%If the backend is not possessed of any special features concerning expectation values, the BackendExpectationValue inheritor only needs to have a single attribute assigned in its definition: BackendCircuitType. the value of this assignment should, of course, be the BackendCircuit inheritor discussed above. \\

%To integrate the backend into \tequila as a whole, the file containing the above extension should be inserted into the tq.simulators folder. Then, the backend should be made accessible by adding imports into the the file \textit{tq.simulators.simulator{\_}api}. Presuming the existence of a package called \textsc{foobar}, which supports sampling, noise, and simulation,is as follows

%\lstinputlisting[language=Python]{code/import_statements.py}

%\subsection{numerical optimizers}

%implementing ones own optimizer will vary in difficulty depending on the complexity and flexibility of the optimizer in question. The classes which must be defined are the inheritors of Optimizer and OptimizerResults. \\

%For the Optimizer inheritor, both the \textit{{\_}{\_}init{\_}{\_}} and \textit{{\_}{\_}call{\_}{\_}} methods must be written. It is recommended to make use of the \textit{initialize{\_}variables} and \textit{compile{\_}objective} methods of the base class. The classmethod \textit{available{\_}methods} should also be defined; this returns a list of all valid strings for accessing method options of the optimizer. See, for example, the implementation of the \tequila GDOptimizer for details.\\

%The OptimizerResults inheritor is fairly simple; other than being defined through the \textsc{dataclass} decorator, it simply need have any unique attributes (such as may be returned by optimization, e.g information returned by the optimization backend directly) defined and given the value None. An instantiated member of this class should be the return value of any calls to the Optimizer inheritor.

%To integrate the new optimizer into \tequila, a wrapper function called \textit{minimize} should be defined. This should instantiate an optimizer, call it, and return whatever the call thereto returns. Finally, the \textit{tq.optimizers.{\_}{\_}init{\_}{\_}.py} file should be altered. In case an external package needs \textsc{Foobar} is being added, then the code added to the imports in the aforementioned file would be as provided below. 

%\lstinputlisting[language=Python]{code/optimizer_import_1.py}

%Additionally, a string representing the optimizer should be added to the list object \textit{SUPPORTED{\_}OPTIMIZERS} near the beginning of the file.

%\subsection{Quantum Chemistry}
%\jsk{pyscf does not work currently}
%At present, \tequila offers plugins for \textsc{PySCF} and \textsc{PSI4}, the two predominant python interfaces for electronic structure calculation. 

